A Regularized Online Newton Method for Stochastic Convex Bandits with Linear Vanishing Noise

We study a stochastic convex bandit problem where the subgaussian noise parameter is assumed to decrease linearly as the learner selects actions closer and closer to the minimizer of the convex loss function. Accordingly, we propose a Regularized Online Newton Method (RONM) for solving the problem, based on the Online Newton Method (ONM) of arXiv:2406.06506. Our RONM reaches a polylogarithmic regret in the time horizon $n$ when the loss function grows quadratically in the constraint set, which recovers the results of arXiv:2402.12042 in linear bandits. Our analyses rely on the growth rate of the precision matrix $\Sigma_t^{-1}$ in ONM and we find that linear growth solves the question exactly. These analyses also help us obtain better convergence rates when the loss function grows faster. We also study and analyze two new bandit models: stochastic convex bandits with noise scaled to a subgaussian parameter function and convex bandits with stochastic multiplicative noise.

==> tex/append/related.tex <==
Initialed by \cite{FK05} and \cite{Kle04}, the literature on convex bandits is increasingly extensive. In the stochastic setting, \cite{AFHK13} first obtained $\operatorname{poly}(d) \sqrt{n}$ regret using classical zeroth-order optimization techniques. Their results were improved by \cite{LG21a}, which yielded a better dependence on dimension. In the adversarial setting, $\sqrt{n}$ regret was also achieved by \cite{HL14} with Online Newton Method  (\textbf{ONM}) when the loss function is both smooth and strongly convex. And if only boundedness of loss function holds, \cite{BDKP15}  showed that $\sqrt{n}$ regret is also possible when the dimension $d=1$. The case for general $d$ was later proved by \cite{BE18}. Their non-constructive information-theoretic via Bayesian minimax duality were followed by \cite{Lat20-cvx}. The current state of art is \textbf{ONM} for which the regret is $d^{3.5}\sqrt{n}$ in the adversarial setting while $d^{1.5}\sqrt{n}$ (informally) in the stochastic setting (\cite{fokkema2024onlinenewtonmethodbandit}).

